3D Video Loops from Asynchronous Input

Looping videos are short video clips that can be looped endlessly without visible seams or artifacts. They provide a very attractive way to capture the dynamism of natural scenes. Existing methods have been mostly limited to 2D representations. In this paper, we take a step forward and propose a practical solution that enables an immersive experience on dynamic 3D looping scenes. The key challenge is to consider the per-view looping conditions from asynchronous input while maintaining view consistency for the 3D representation. We propose a novel sparse 3D video representation, namely Multi-Tile Video (MTV), which not only provides a view-consistent prior, but also greatly reduces memory usage, making the optimization of a 4D volume tractable. Then, we introduce a two-stage pipeline to construct the 3D looping MTV from completely asynchronous multi-view videos with no time overlap. A novel looping loss based on video temporal retargeting algorithms is adopted during the optimization to loop the 3D scene. Experiments of our framework have shown promise in successfully generating and rendering photorealistic 3D looping videos in real time even on mobile devices. The code, dataset, and live demos are available in https://limacv.github.io/VideoLoop3D_web/.

==> figs_tabs/metrics_comp.tex <==
% \begin{table*}[t]
% \centering
% \begin{tabular}{l|ccccc|ccc}
%     & \textit{VLPIPS}$\downarrow$  & \textit{STDerr}$\downarrow$  & \textit{Com.}$\downarrow$  & \textit{Coh.}$\downarrow$  & \textit{LoopQ}$\downarrow$ & \textit{\# Params.}$\downarrow$ & \textit{Render Spd}$\uparrow$ & \textit{Train Time}$\downarrow$\\ 
% \hline
% Ours          & \textbf{0.1392} & \textbf{56.02} & \textbf{10.65} & \textbf{9.269} & \textbf{9.263} & \multirow{2}{*}{20M-89M} & \multirow{2}{*}{\textbf{140fps}} &  \multirow{2}{*}{\textbf{~3h}}\\
% loop2D + MTV    & 0.2447 & 118.9 & 11.83 & 9.919 & 9.927 & & & \\
% loop2D + MPV    & 0.2546 & 117.5 & 11.82 & 9.817 & 9.840 & 1060M & 110fps & 27.22GB  \\
% loop2D + DyNeRF & 0.2282 & 123.7 & 11.93     & 10.23 & 10.27  & \textbf{2M} & 0.1fps & 3168GB \footnotemark \\ 
% \hline
% \end{tabular}
% \caption{Quantitative comparison in terms of reconstruct quality and efficiency. $\downarrow$ indicates lower is better and vice versa. We bold the \textbf{best} for each item. Our method achieves the best performance and strike a balance between number of parameters and render speed. }
% \label{tab:comp}
% \end{table*}
